Interprocedural Semantic Change-Impact Analysis using Equivalence Relations

Change-impact analysis (CIA) is the task of determining the set of program elements impacted by a program change. Precise CIA has great potential to avoid expensive testing and code reviews for (parts of) changes that are refactorings (semantics-preserving). Existing CIA is imprecise because it is coarse-grained, deals with only few refactoring patterns, or is unaware of the change semantics. We formalize the notion of change impact in terms of the trace semantics of two program versions. We show how to leverage equivalence relations to make dataflow-based CIA aware of the change semantics, thereby improving precision in the presence of semantics-preserving changes. We propose an anytime algorithm that allows applying costly equivalence relation inference incrementally to refine the set of impacted statements. We have implemented a prototype in SymDiff, and evaluated it on 322 real-world changes from open-source projects and benchmark programs used by prior research. The evaluation results show an average 35% improvement in the size of the set of impacted statements compared to standard dataflow-based techniques.

==> algo.tex <==
% !TEX root = main.tex

\begin{algorithm}
 \KwIn{$<V, V'>$, changed\_procedures : proc $\times$ proc}
 \KwOut{Impacted Statements}
  $T \longleftarrow DCF(changed\_procedures_{|1}, V)$;\\
  $T' \longleftarrow DCF(changed\_procedures_{|2}, V')$;\\
  $EQ \longleftarrow \{x = x' | x \not\in T \land x' \not\in T'\}$;\\
  $EQ \longleftarrow SymDiff^{+}(V, V', EQ)$;\\
  $T \longleftarrow DCF_E(changed\_procedures_{|1}, V, EQ)$;\\
  $T' \longleftarrow DCF_E(changed\_procedures_{|2}, V', EQ)$;\\
   
 \caption{Naive algorithm}
 \label{alg:naive}
\end{algorithm}

==> diff.tex <==
% !TEX root = main.tex
\appendix{Inferring Equalities}
\label{sec:diff}

\Fix{Move this to appendix or implementation.}

%In previous section, we assumed an oracle \InferEq that computes $\preEqn$ and $\summEqn$ given $\program{1}$ and $\program{2}$.
In this section, we will describe one particular implementation of $\preEqn$ and $\summEqn$ using a product construction in \SymDiff{}~\cite{lahiri-fse13}.
We choose the product construction in \SymDiff{} because it allows for precise interprocedural differential reasoning over the product of two programs; most other product constructions are limited to single procedures with loops.
We start by briefly summarizing the product construction (detailed description is outside the scope of this work) and the inference of equivalences over the product. 
We next identify restrictions under which these equivalences serve as valid $\preEqn$ and $\summEqn$ and augment the product construction to ensure these restrictions. 

% Given P1, P2
% For each f \in Procs
%   Construct MS_f^1_f^2 (f^1 \in Procs^1, ..)
%      - input is x^1, x^2, output is y^1, y^2
%      - body  inline_f^1, inline_f^2, constrain
%      - each call is instrumened as:
%          in_g_i = e1, out_g_i = r1, taken_g_i =  true
%      - constrain = 
%             if (taken_g_i && taken_g'_j) 
%                 call r1, r2 = MS_g_g'(in_, ..);
%                 assume out1 == r1 ..
%      - cand pre (x == x'), cand post (y == y'), cand post summeq_post
%          Candidates {x == x', y == y', (\and_x {\depends{y, x, f}} x == x') ==> y == y'}
%      - pre (x == x') for MS_main_main'
%
%  Thm: If summeq_post is inferred, then summeq(y) holds


\subsection{Product Program Construction}
\label{sec:product}

% \begin{figure}[tb]
% \begin{lstlisting}[language=boogie,numbers=left,xleftmargin=2.5em,frame=lines,mathescape=true]
% proc $\prodProc{\pproc}{1}{2}$($\vect{\varn{x}}^1$, $\vect{\varn{x}}^2$): ($\vect{\varn{r}}^1$, $\vect{\varn{r}}^2$)
% {
%     //-- initialize call sequences ---
%     var $\takenProc{1}, \takenProc{2}$ := $\emptyset, \emptyset$; %\label{line:dac-init}%
%     //-- Start of $\pproc^1$ body %\label{line:dac-proc1-start}%
%     ...
%     $\inputAt{\altproc{}}{\procNode{1}}{1}$ := $\vect{e}^1$; // record inputs %\label{line:dac-v1call-in}%
% $\procNode{1}$: %\underline{\textbf{call} $\vect{\varn{r}}^1$ := $\altproc{}^1(\vect{e}^1)$;}%  %\label{line:dac-v1call}%
%     $\takenProc{1}$ += $(\procNode{1}, \altproc{}, \vect{e}^1, \vect{\varn{r}}^1)$;  // record call %\label{line:dac-v1call-csite}%
%     %%$\outputAt{\altproc{}}{\procNode{1}}{1}$:= $r^1$;    //record output %\label{line:dac-v1call-out}%
%     ...
%     //End of $\pproc^1$ body %\label{line:dac-proc1-end}%
%     //-- Start of $\pproc^2$ body %\label{line:dac-proc2-start}%
%     ...
%     $\inputAt{\hproc}{\procNode{2}}{2}$ := $\vect{e}^2$; // record inputs %\label{line:dac-v2call-in}%
% $\procNode{2}$: %\underline{\textbf{call} $\vect{\varn{r}}^2$ := $\hproc^2(\vect{e}^2)$;}%  %\label{line:dac-v1call}%
%     $\takenProc{2}$ += $(\procNode{2},\hproc)$;     // record callsite %\label{line:dac-v2call-csite}%
%     $\outputAt{\hproc}{\procNode{2}}{2}$ := $r^2$;    //record output %\label{line:dac-v2call-out}%
%     ...    
%     //End of $\pproc^2$ body %\label{line:dac-proc2-end}%
%     //-- constrain calls
%     foreach (var $\altproc{}$ in $\Procs{}$) {  %\label{line:dac-loop1}%
%       foreach ($(\procNode{i}, \altproc{})$ in $\takenProc{1}$) { %\label{line:dac-loop2}%
%          foreach ($(\procNode{j}, \altproc{})$ in $\takenProc{2}$) {  %\label{line:dac-loop3}%
%             //replay inputs
%             call $o^1, o^2$ := $\prodProc{\aaltproc}{1}{2}$($\inputAt{\altproc{}}{\procNode{i}}{1}$, $\inputAt{\altproc{}}{\procNode{j}}{2}$); %\label{line:dac-call-product}%
%             //constrain outputs
%             assume ($o^1 == \outputAt{\altproc{}}{\procNode{i}}{1} \wedge o^2 == \outputAt{\altproc{}}{\procNode{j}}{2}$); %\label{line:dac-constrain-product}%
%          }
%       }
%     } %\label{line:dac-loop1-end}%
%     $\highlight{\bassert \takenProc{1} ==_{\textit{procs}} \takenProc{2}}$; 
%     return;
% }

% proc $\prodProc{\mainProc}{1}{2}$($\vect{\varn{x}}^1$, $\vect{\varn{x}}^2$)
% free requires  $\vect{\varn{x}}^1 == \vect{\varn{x}}^2$
% {
% ...
% }
% \end{lstlisting}
% \caption{Product procedures for inferring equivalences~\cite{lahiri-fse13a}.}
% \label{fig:product-program}
% \end{figure}


\begin{figure}[tb]
\begin{lstlisting}[language=boogie,numbers=left,xleftmargin=2.5em,frame=lines,mathescape=true]
proc $\prodProc{\pproc}{1}{2}$($\vect{\varn{x}}^1$, $\vect{\varn{x}}^2$): ($\vect{\varn{r}}^1$, $\vect{\varn{r}}^2$)
{
    //-- initialize call sequences ---
    var $\takenProc{1}, \takenProc{2}$ := $\emptyset, \emptyset$; %\label{line:dac-init}%
    //-- Start of $\pproc^1$ body %\label{line:dac-proc1-start}%
    ...
$\procNode{1}$: %\underline{\textbf{call} $\vect{\varn{r}}^1$ := $\altproc{}^1(\vect{e}^1)$;} //$\vect{\varn{r}}^1 \cap \readSet{\vect{e}^1} = \emptyset$ %  %\label{line:dac-v1call}%
    $\takenProc{1}$ += $(\procNode{1}, \altproc{}, \vect{e}^1, \vect{\varn{r}}^1)$;  // record call %\label{line:dac-v1call-csite}%
    ...     
    //-- End of $\pproc^1$ body %\label{line:dac-proc1-end}% 
    //-- Start of $\pproc^2$ body %\label{line:dac-proc2-start}%
    ...
$\procNode{2}$: %\underline{\textbf{call} $\vect{\varn{r}}^2$ := $\hproc^2(\vect{e}^2)$;} //$\vect{\varn{r}}^2 \cap \readSet{\vect{e}^2} = \emptyset$ %  %\label{line:dac-v2call}%
    $\takenProc{2}$ += $(\procNode{2}, \altproc{}, \vect{e}^2, \vect{\varn{r}}^2)$;  // record call %\label{line:dac-v2call-csite}%
    ...    
    //-- End of $\pproc^1$ body %\label{line:dac-proc2-end}%  
    //-- constrain calls
    foreach (var $\altproc{}$ in $\Procs{}$) {  %\label{line:dac-loop1}%
      foreach ($(\procNode{i}, \altproc{}, \vect{e}^1, \vect{\varn{y}}^1)$ in $\takenProc{1}$) { %\label{line:dac-loop2}%
         foreach ($(\procNode{j}, \altproc{}, \vect{e}^2, \vect{\varn{y}}^2)$ in $\takenProc{2}$) {  %\label{line:dac-loop3}%
            //replay inputs
            call $\vect{\varn{o}}^1, \vect{\varn{o}}^2$ := $\prodProc{\aaltproc}{1}{2}$($\vect{e}^1$, $\vect{e}^2$); %\label{line:dac-call-product}%
            //constrain outputs
            assume ($\vect{\varn{o}}^1 == \vect{\varn{y}}^1 \wedge \vect{\varn{o}}^2 == \vect{\varn{y}}^2 $); %\label{line:dac-constrain-product}%
         }
      }
    } %\label{line:dac-loop1-end}%
    $\highlight{\bassert \takenProc{1} ==_{\textit{procs}} \takenProc{2}}$; %\label{line:dac-modification}%
}
proc $\prodProc{\mainProc}{1}{2}$($\vect{\varn{x}}^1$, $\vect{\varn{x}}^2$)
free requires  $\vect{\varn{x}}^1 == \vect{\varn{x}}^2$
{ ... }
\end{lstlisting}
\caption{Product procedures for inferring equivalences~\cite{lahiri-fse13}.}
\label{fig:product-program}
\vspace{\vsp}
\end{figure}


Given $\program{1}$ and $\program{2}$, \SymDiff{} generates a product program $\prodProg{1}{2}$ that defines a procedure $\prodProc{\pproc}{1}{2}$ for every $\pproc \in \Procs{}$.
Loops are already assumed to be extracted as tail-recursive procedures in $\Procs{}$. 
Figure~\ref{fig:product-program} shows the high-level structure of a product procedure; we will ignore the highlighted statement for now.  
The input and output formals of $\prodProc{\pproc}{1}{2}$ is a concatenation of the inputs and outputs of $\pproc^1$ and $\pproc^2$, suitably renamed. 
The body of $\prodProc{\pproc}{1}{2}$ consists of 3 parts.
(1) Line~\ref{line:dac-init} initializes two variables $\takenProc{i}$ that capture the sequence of callsites in a trace through the body of $\pproc^i$.
(2) Lines~\ref{line:dac-proc1-start},\ldots,\ref{line:dac-proc1-end} and Lines~\ref{line:dac-proc2-start},\ldots,\ref{line:dac-proc2-end}  contain the bodies of $\pproc^1$ and $\pproc^2$ respectively.
Any callsite in either $\pproc^i$ (underlined) is instrumented to track (a) the arguments  (b) returns and (c) callsite (e.g. line~\ref{line:dac-v1call-csite}).
(3) Finally, lines~\ref{line:dac-loop1},\ldots,~\ref{line:dac-loop1-end} iterate through all pair of callsites in a path in $\pproc^1$ and $\pproc^2$ with the same callee (say $\aaltproc$), and invokes the product procedure $\prodProc{\aaltproc}{1}{2}$ with corresponding arguments (line~\ref{line:dac-call-product}, and constrains the outputs to be outputs from the respective callsites (line~\ref{line:dac-constrain-product}). 
%
The product procedure $\prodProc{\mainProc}{1}{2}$ that is the entry procedure for $\prodProg{1}{2}$ has a precondition to constrain the input arguments $\vect{\varn{x}}^1$ and $\vect{\varn{x}}^2$ to start in equal states.

For a procedure $\pproc$ with inputs $\vect{\varn{x}}$ and outputs $\vect{\varn{r}}$, a Boolean expression $\phi(\vect{\varn{x}}) \Rightarrow \psi(\vect{\varn{x}}, \vect{\varn{r}})$ is a {\it summary} for $\pproc$ if for any $(\store{1},\store{2}) \in \transRel{\pproc}$, if $\store{1}$ satisfies $\phi$, then $\store{2}$ satisfies $\psi$.
The following theorem relates $\prodProc{\pproc}{1}{2}$ with $\pproc^1$ and $\pproc^2$.
\begin{theorem}[~\cite{lahiri-fse13}]
If $\phi(\vect{\varn{x}}^1, \vect{\varn{x}}^2) \Rightarrow \psi(\vect{\varn{x}}^1, \vect{\varn{x}}^2, \vect{\varn{r}}^1, \vect{\varn{r}}^2)$ is a summary for a product procedure $\prodProc{\pproc}{1}{2}$, then
%\begin{quote}
for any $(\store{1},\store{2}) \in \transRel{\pproc}^1$ and $(\store{3},\store{4}) \in \transRel{\pproc}^2$, if $\storeUnion{\store{1}}{\store{3}}$ satisfies $\phi$ then $\storeUnion{\store{2}}{\store{4}}$ satisfies $\psi$. 
%\end{quote}
\end{theorem}

\subsection{Equivalence inference}
For the product program $\prodProg{1}{2}$, one can leverage any of the (single program) invariant generation techniques based on abstract-interpretation~\cite{cousot-popl77}, or interpolants~\cite{mcmillan-tacas04} to infer preconditions, postconditions (including two-state postconditions) on $\prodProc{\pproc}{1}{2}$.
Such invariants are {\it relational} or {\it differential} in that they are over the state of two programs $\program{1}$ and $\program{2}$. 
Equivalences are special classes of such relational invariants and therefore we leverage the invariant generation over $\prodProg{1}{2}$ to infer $\preEqn$ and $\summEqn$.
In the next few paragraphs, we identify conditions under which such relational invariants can yield our desired equivalences.

%\subsubsection{Inferring $\summEqn$}

% 
% SUMM_EQUAL
% ----------------
%  theorem
% 

%% summary predicate

For an output formal $\varn{r} \in \ProcOuts{\pproc}$, let $\summPredicate{\varn{r}^1}{\varn{r}^2}$ be the predicate $
\left(\bigwedge_{\varn{x} \in \ProcIns{\pproc} \text{ and } \varn{x} \in \dependencyOf{\varn{r}}} \varn{x}^1 == \varn{x}^2\right)
\Rightarrow \varn{r}^1 == \varn{r}^2 
$.

\begin{theorem}
For a product program $\prodProg{1}{2}$ and a procedure $\prodProc{\pproc}{1}{2}$ and  output parameter $\varn{r} \in \ProcOuts{\pproc}$, if $\summPredicate{\varn{r}^1}{\varn{r}^2}$ is a summary of $\prodProc{\pproc}{1}{2}$, then $\summEq{\varn{r}}{\pproc}$ holds, provided all executions in $\pproc^1$ and $\pproc^2$ are terminating.
\end{theorem}

%\Shuvendu{Say why we need the termination, and relaxation to equitermination}

%
%  However: pre is inferred =/=> preEq hold
%         - equitermination ((s, ne_f, empty) --*--> (t, nx_f, empty) <==> (s, ne_f', empty) --*--> (t', nx_f', empty)
%         - different call-return history on each input from main
%         - refer to exampke
%
%  Assume these. Point to plausible solutions (mutual termination/relative termination and history sequence)
%
%       if all the CSpost assertions are proved, and the P1, P2 are equiterminating, 
%             pre inferred ==> preEq 

% Adding freeEq from EQ
% Dropping procedures from Prog1, Prog2
% - we drop candidates, depending on other callsites
% - drop post if no body

% OPTIONAL               
%  For equitermination, we can investigate mutual termination/relative termination
%  Here we focs on diferent history, assuming equitermination/termination
%
%  To ensure that each procedure is called in the same seq
%       add a input variable cs and output variable cs' of type seq<procedures>
%       call x := g(y) --> call x := g(y); taken_g_{i++}; cs = cs + g;
%       add CSpost::post cs_in == cs_in' => cs_out == cs_out'
%       if all the CSpost assertions are proved, and the P1, P2 are equiterminating, 
%             pre inferred ==> preEq 
%
% 



%\subsubsection{Inferring $\preEqn$}

\begin{theorem}
For a product program $\prodProg{1}{2}$ and a procedure $\prodProc{\pproc}{1}{2}$ and  input parameter $\varn{x} \in \ProcIns{\pproc}$, if $\varn{x}^1 == \varn{x}^2$ is a precondition of $\prodProc{\pproc}{1}{2}$, then $\preEq{\varn{x}}{\pproc}$ holds, provided: 
\begin{enumerate}
\item All executions in $\program{1}$ and $\program{2}$ are terminating,
\item For any procedure $\hproc \in \Procs{}$, and for any pair of traces $\ProcTracesStarting{\hproc}{\sstore}{1}$ and $\ProcTracesStarting{\hproc}{\sstore}{2}$ starting in $\sstore$, the sequences of procedures calls are identical.
\end{enumerate}
\label{thm:preEqSymdiff}
\end{theorem}

\begin{figure}[h!]
\begin{minipage}[t]{0.2\textwidth}
\begin{lstlisting}[style=C-github,mathescape=true,numbers=none]
void $\mainProc$() 
{
  $\proc{}$(1, 2);
}
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.25\textwidth}
\begin{lstlisting}[style=C-github,mathescape=true,numbers=none]
int $\proc{}$(int x, int y)
{
  int r = x + 2; 
@a@+ (*@{\btHL[fill=gitadd]$\proc{}$}@*)(r, y);@a@
  return r;
}
\end{lstlisting}
\end{minipage}
\caption{Example illustrating side conditions for inference.}
\label{fig:unsound-pre-summ}
\vspace{\vsp}
\end{figure}


\begin{paragraph}{Example} Figure~\ref{fig:unsound-pre-summ} illustrates the need for the side conditions when working with the product program.~\Fix{which side condition? unclear.}
The change in $\proc{}$ adds an infinite loop in $\program{2}$ by calling itself. 
Here $\dependencyOf{\varn{r}} = \{\varn{x}\}$ for $\proc{}$ in both programs. 
Since $\proc{}$ does not terminate, neither does $\prodProc{\pproc}{1}{2}$. 
Hence, $(\varn{x}^1 == \varn{x}^1) \Rightarrow \varn{r}^1 == \varn{r}^2$ is a vacuous summary of $\prodProc{\pproc}{1}{2}$, although $\summEq{\varn{y}}{\pproc}$ does not hold.
%
On the other hand, since $\pproc{}$ does not invoke itself in $\program{1}$, no calls to $\prodProc{\pproc}{1}{2}$ are made from within $\prodProc{\pproc}{1}{2}$. 
This means that $\varn{x}^1 == \varn{x}^2$ is a precondition for $\prodProc{\pproc}{1}{2}$, although $\preEq{\varn{x}}{\pproc}$ does not hold.
% since the $\pproc$ is visited infinitely in $\program{2}$ and only once in $\program{1}$ on the only trace from $\mainProc$. 
\end{paragraph}

Termination is a desirable property for a program and can be verified separately (e.g. establishing ranking functions for loops and recursive procedures.
In fact, we can relax the need for every execution to terminate by only requiring {\it equitermination} (an input $\sstore$ leads to a terminating execution in $\program{1}$ if an only if $\program{2}$ terminates on the same input)~\cite{hawblitzel-cade13}; this is an area of future work. 
For this work, we (unsoundly) assume that the changes do not introduce or fix non-termination. 

Satisfying the second side condition for Theorem~\ref{thm:preEqSymdiff}, unfortunately, cannot be reduced to a standard program verification task.
We informally describe a modification to the product construction (Figure~\ref{fig:product-program}) that provides a sufficient check for ensuring that call sequences from a common input are identical.
We reuse the history variables $\takenProc{i}$ that  capture the call sequences along any path in either procedures (lines~\ref{line:dac-v1call-csite} and~\ref{line:dac-v2call-csite}).
We add an assertion (highlighted in line~\ref{line:dac-modification}) that checks if call sequence through $\pproc^1$ is identical to $\pproc^2$ (assuming equitermination);
the equality $==_{\textit{procs}}$ compares the two sequences after projecting on to the second element (procedure name) of each tuple. 
If {\it every} product procedure satisfies this assertion, starting from only the assumption that arguments to $\mainProc$ are identical, then one can ensure the second side condition for Theorem~\ref{thm:preEqSymdiff}.
Our implementation currently does not handle this modification. 

% \subsection{Incorporating additional equalities}
% Recall that the procedure \InferEq (Algorithm~\ref{algo:anytime}) takes as input a set of equalities $(\preqs,\summeqs)$ that are guaranteed to hold by dataflow analysis.
% These facts are added as assumptions on the product program $\prodProg{1}{2}$ as follows:
% %\begin{itemize}
% %\item 
% If $(\varn{x}, \pproc) \in$ $\preqs$ (resp. $\summeqs$) then we add an {\it free} (unchecked) precondition  $\varn{x}^1 == \varn{x}^2$ (resp. postcondition $\summPredicate{\varn{x}^1}{\varn{x}^2}$) to $\prodProc{\pproc}{1}{2}$.
% These facts help the inference algorithm to converge faster by pruning the search space and avoiding to infer these equivalences.


% Note that equiterminating condition subsumes cases where the two programs are loop and recursion free.


% Unfortunately, a similar property does not hold for preconditions of the product procedures.

% \begin{quote}
% For the product program $\prodProg{1}{2}$, for any  product procedure $\prodProc{\proc{}}{1}{2}$ and  input parameters $\varn{x}^1 \in \ProcIns{\proc{}}^1, \varn{x}^2 \in \ProcIns{\proc{}}^2$,  $\varn{x}^1 == \varn{x}^2$ may be precondition of $\prodProc{\proc{}}{1}{2}$, but $\preEq{\varn{x}}$ may not hold. 
% \end{quote}



% %
% %
% % IN_PARAM_EQUAL
% % ----------------
% %   unsoundness for equitermination
% %   unsoundness for different history
% % 
% %  theorem
% %
% %    
% %
 

% \begin{figure}[h!]
% \begin{minipage}[t]{0.2\textwidth}
% \begin{lstlisting}[language=boogie,mathescape=true]
% proc $\mainProc$() 
% {
%   call $\proc{1}$(0);
%   //extra call to $\proc{1}$  
%   + call $\proc{1}$(0); 
% }
% \end{lstlisting}
% \end{minipage}
% \begin{minipage}[t]{0.25\textwidth}
% \begin{lstlisting}[language=boogie,mathescape=true]
% proc $\proc{1}$(x:int) 
% {
%   - call $\proc{2}$(1);
%   //different arg to $\proc{2}$
%   + call $\proc{2}$(2); 
%   assume false;
% }
% \end{lstlisting}
% \end{minipage}    
% \caption{Examples illustrating unsoundness of inference of $\preEqn$}
% \label{fig:unsound-preeq}
% \end{figure}

% \Shuvendu{Describe conditions under which the preconditions are sound mutual preconditions}

% Figure~\ref{fig:unsound-preeq} shows two main conditions under which a valid precondition of the product program fails to be a $\preEqn$.
% \begin{enumerate}
% \item $\varn{x}^1 == \varn{x}^2$ is a valid precondition for $\prodProc{\proc{1}}{1}{2}$ because all the call sites (in either program) invoke $\proc{1}$ with argument $0$ for $\varn{x}$. 
% However, in $\program{1}$, the (only) execution from $\mainProc$ has exactly one occurrence $\proc{1}$, whereas the execution in $\program{2}$ invokes $\proc{1}$ twice. 
% Therefore projecting the executions on the entry node of $\proc{1}$ will yield sequences of size 1 and 2 respectively; thus $\preEq{\varn{x}}$ does not hold by definition. 
% \item $\varn{x}^1 == \varn{x}^2$ is a valid precondition for $\prodProc{\proc{2}}{1}{2}$ because of {\it non-termination}.
% The callsite for $\prodProc{\proc{2}}{1}{2}$ is reachable only for terminating executions of $\prodProc{\proc{1}}{1}{2}$.
% However, the $\bassume{\bfalse}$ makes such a set empty, and thus the precondition holds vacuously.
% \end{enumerate}

% \subsubsection{Equitermination}
% To remedy termination, we can resort to loop/recursion free programs.
% A more general criteria is to check that each procedure equiterminates using Mutual Termination~\cite{godlin-mutual-termination} or Relative Termination~\cite{hawblitzel-cade13}.
% \Shuvendu{Elaborate?}

% \subsubsection{Same call sequence}
% We need to ensure that for a given input state, all the call sequences on the two programs are identical.
% A sufficient way to ensure this is that each procedure witnesses the same terminating call sequences, starting at states that are related.
% This can be ensured that the call sequences within a procedure are identical. 
% \Shuvendu{If we have any change that impacts control flow, then this check will fail.}
% The highlighted assertion in Figure~\ref{fig:product-program} expresses this check, where $\takenProc{1} ==_\textit{procs} \takenProc{2}$ denotes equality of the procedure components in the two sequence. 

% \begin{theorem}
% For the product program $\prodProg{1}{2}$, if (a) the two programs are equiterminating, and (b)  the highlighted assertions in $\prodProc{\proc{}}{1}{2}$ holds for each procedure $\proc{} \in Procs{}$, and $\varn{x}^1 == \varn{x}^2$ is a precondition for $\prodProc{\altproc{}}{1}{2}$, then $\preEq{\varn{x}}{\altproc{}}$ holds.
% \end{theorem}
% Note that equiterminating condition subsumes cases where the two programs are loop and recursion free.

% \Shuvendu{Any impacted variable that determines if a call happens will destroy the premise of this restriction.}

% %


%\subsection{Inlining}

%\Shuvendu{Show a simple example of null extraction from callee to caller}

% \Alex{Describe the example that illustrates benefit of inlining here (shuvendu)}

% The example in \fig~\ref{fig:inline-example-c} shows an example where the developer decides to remove a redundant check in the function getSize. The example shows a simplified snippet of a worklist algorithm using a deque. The loop executes until the deque is empty. The call to process could add elements to the deque.
% The emtpy check on the deque is made by checking the size is greater than 0, but the procedure computing the size first checks whether the argument is \codein{NULL}. This check is redundant here. 

% \input{inlining_example}

\appendix{Anytime Algorithm}

It  is worth highlighting that small bounds for $k$ may not always suffice to achieve precise results, as illustrated by the example in Figure~\ref{fig:examples-anytime-2}.
For this example $\changedProcs = \{\mainProc\}$; 
%$\proc{1}$ has two call sites, one in $\mainProc$ and the other in $\proc{2n}$. 
The set $\kChangedProcs$ grows as follows across iterations: $\{\mainProc\}$, 
$\{\proc{2n}, \mainProc, \proc{1}\}$, $\{\proc{2n-1}, \proc{2n}, \mainProc, \proc{1}, \proc{2}\}$, and so on.
It is not hard to see that until $\kChangedProcs = \Procs{}$, \InferEq will not be able to infer that the $\preEq{\varn{x}}{\proc{1}}$ holds.
\Fix{Move this example and Figure 5 to extended report and add a link}
%This equivalence relies on discovering $\preEq{\varn{x}}{\proc{2n}}$, which in turn depends on $\preEq{\varn{x}}{\proc{2n-1}}$, and eventually depends on $\preEq{\varn{x}}{\proc{1}}$.
%To establish this compositionally, we need to analyze the entire program. 


\begin{figure}[h!]
\begin{minipage}[t]{0.20\textwidth}
\begin{lstlisting}[style=C-github,mathescape=true,numbers=none]
void $\mainProc$(int x) 
{
@d@- (*@{\btHL[fill=gitdel]$\proc{1}$}@*)(x);@d@ 
@a@+ (*@{\btHL[fill=gitadd]$\proc{1}$}@*)(x@af@+0@af@);@a@
}
void $\proc{1}$(int x) 
{
  $\proc{2}$(x+1);
}
...
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.25\textwidth}
\begin{lstlisting}[style=C-github,mathescape=true,numbers=none]
void $\proc{2n-1}$(int x) 
{
  $\proc{2n}$(x+2n-1);
}
void $\proc{2n}$(int x) 
{
  if (x > 0)
    $\proc{1}$(x-1);
}
\end{lstlisting}
\end{minipage}
\caption{Pathological example that needs large $k$}
\label{fig:examples-anytime-2}
\vspace{\vsp}
\end{figure}




==> inlining_example.tex <==
% !TEX root = main.tex

\begin{figure}[tb]
{\small{
\begin{lstlisting}[language=C,frame=lines]
int getSize(t_deque* st) {
  // The change here is to remove the if, and the return -1. 
  //The else branch is unfeasible here so no point in keeping it.
  if (st != NULL)
    return (st->tail - st->head) & (st->length - 1);
  return -1;
}

int doWork(t_deque *st) {
  if (st != NULL) {
    int elem;
    // This call site should not be impacted
    if (getSize(st) > 0 && elem = deque(st)) {
      process(elem, st);
      return doWork(st);
    }
    return 0;
  }
  return -1;
}

...
void perform(t_deque *st) {
  //This call site should be impacted
  getSize(t_deque* st);
  ...
}

\end{lstlisting}
}}
\caption{C program motivating inlining}
\label{fig:inline-example-c}
\vspace{\vsp}
\end{figure}



==> scripts/results_dac_linear_table.tex <==
% !TEX root = ../main.tex

\begin{figure*}[tb]
\begin{center}
\small
\begin{tabular}{l||rrr|rr}
\toprule
Project & Change Size & Syntactic & Semantic & Synt Time & Sem Time\\
\midrule
\Use{ProjectName}&\Use{ProjectChangeSize}&\Use{ProjectSyntacticLines}&\Use{ProjectSemanticLines}&\Use{ProjectSyntacticTime}&\Use{ProjectSemanticTime}\\
\Use{histo_20a156Name}&\Use{histo_20a156ChangeSize}&\Use{histo_20a156SyntacticLines}&\Use{histo_20a156SemanticLines}&\Use{histo_20a156SyntacticTime}&\Use{histo_20a156SemanticTime}\\
\Use{histo_3439beName}&\Use{histo_3439beChangeSize}&\Use{histo_3439beSyntacticLines}&\Use{histo_3439beSemanticLines}&\Use{histo_3439beSyntacticTime}&\Use{histo_3439beSemanticTime}\\
\Use{histo_4a6f2aName}&\Use{histo_4a6f2aChangeSize}&\Use{histo_4a6f2aSyntacticLines}&\Use{histo_4a6f2aSemanticLines}&\Use{histo_4a6f2aSyntacticTime}&\Use{histo_4a6f2aSemanticTime}\\
\Use{histo_6a5d36Name}&\Use{histo_6a5d36ChangeSize}&\Use{histo_6a5d36SyntacticLines}&\Use{histo_6a5d36SemanticLines}&\Use{histo_6a5d36SyntacticTime}&\Use{histo_6a5d36SemanticTime}\\
\Use{histo_96635dName}&\Use{histo_96635dChangeSize}&\Use{histo_96635dSyntacticLines}&\Use{histo_96635dSemanticLines}&\Use{histo_96635dSyntacticTime}&\Use{histo_96635dSemanticTime}\\
\Use{histo_c4efeeName}&\Use{histo_c4efeeChangeSize}&\Use{histo_c4efeeSyntacticLines}&\Use{histo_c4efeeSemanticLines}&\Use{histo_c4efeeSyntacticTime}&\Use{histo_c4efeeSemanticTime}\\
\Use{histo_c723a4Name}&\Use{histo_c723a4ChangeSize}&\Use{histo_c723a4SyntacticLines}&\Use{histo_c723a4SemanticLines}&\Use{histo_c723a4SyntacticTime}&\Use{histo_c723a4SemanticTime}\\
\Use{histo_fb8f50Name}&\Use{histo_fb8f50ChangeSize}&\Use{histo_fb8f50SyntacticLines}&\Use{histo_fb8f50SemanticLines}&\Use{histo_fb8f50SyntacticTime}&\Use{histo_fb8f50SemanticTime}\\
\Use{dyad_014373Name}&\Use{dyad_014373ChangeSize}&\Use{dyad_014373SyntacticLines}&\Use{dyad_014373SemanticLines}&\Use{dyad_014373SyntacticTime}&\Use{dyad_014373SemanticTime}\\
\Use{dyad_0321ebName}&\Use{dyad_0321ebChangeSize}&\Use{dyad_0321ebSyntacticLines}&\Use{dyad_0321ebSemanticLines}&\Use{dyad_0321ebSyntacticTime}&\Use{dyad_0321ebSemanticTime}\\
\Use{dyad_05c663Name}&\Use{dyad_05c663ChangeSize}&\Use{dyad_05c663SyntacticLines}&\Use{dyad_05c663SemanticLines}&\Use{dyad_05c663SyntacticTime}&\Use{dyad_05c663SemanticTime}\\
\Use{dyad_0b67eaName}&\Use{dyad_0b67eaChangeSize}&\Use{dyad_0b67eaSyntacticLines}&\Use{dyad_0b67eaSemanticLines}&\Use{dyad_0b67eaSyntacticTime}&\Use{dyad_0b67eaSemanticTime}\\
\Use{dyad_23b39eName}&\Use{dyad_23b39eChangeSize}&\Use{dyad_23b39eSyntacticLines}&\Use{dyad_23b39eSemanticLines}&\Use{dyad_23b39eSyntacticTime}&\Use{dyad_23b39eSemanticTime}\\
\Use{dyad_243b6bName}&\Use{dyad_243b6bChangeSize}&\Use{dyad_243b6bSyntacticLines}&\Use{dyad_243b6bSemanticLines}&\Use{dyad_243b6bSyntacticTime}&\Use{dyad_243b6bSemanticTime}\\
\Use{dyad_275412Name}&\Use{dyad_275412ChangeSize}&\Use{dyad_275412SyntacticLines}&\Use{dyad_275412SemanticLines}&\Use{dyad_275412SyntacticTime}&\Use{dyad_275412SemanticTime}\\
\Use{dyad_33e5c3Name}&\Use{dyad_33e5c3ChangeSize}&\Use{dyad_33e5c3SyntacticLines}&\Use{dyad_33e5c3SemanticLines}&\Use{dyad_33e5c3SyntacticTime}&\Use{dyad_33e5c3SemanticTime}\\
\Use{dyad_3d7f0cName}&\Use{dyad_3d7f0cChangeSize}&\Use{dyad_3d7f0cSyntacticLines}&\Use{dyad_3d7f0cSemanticLines}&\Use{dyad_3d7f0cSyntacticTime}&\Use{dyad_3d7f0cSemanticTime}\\
\Use{dyad_3dfc1bName}&\Use{dyad_3dfc1bChangeSize}&\Use{dyad_3dfc1bSyntacticLines}&\Use{dyad_3dfc1bSemanticLines}&\Use{dyad_3dfc1bSyntacticTime}&\Use{dyad_3dfc1bSemanticTime}\\
\Use{dyad_4f2360Name}&\Use{dyad_4f2360ChangeSize}&\Use{dyad_4f2360SyntacticLines}&\Use{dyad_4f2360SemanticLines}&\Use{dyad_4f2360SyntacticTime}&\Use{dyad_4f2360SemanticTime}\\
\Use{dyad_52d97aName}&\Use{dyad_52d97aChangeSize}&\Use{dyad_52d97aSyntacticLines}&\Use{dyad_52d97aSemanticLines}&\Use{dyad_52d97aSyntacticTime}&\Use{dyad_52d97aSemanticTime}\\
\Use{dyad_5eeb47Name}&\Use{dyad_5eeb47ChangeSize}&\Use{dyad_5eeb47SyntacticLines}&\Use{dyad_5eeb47SemanticLines}&\Use{dyad_5eeb47SyntacticTime}&\Use{dyad_5eeb47SemanticTime}\\
\Use{dyad_7fc140Name}&\Use{dyad_7fc140ChangeSize}&\Use{dyad_7fc140SyntacticLines}&\Use{dyad_7fc140SemanticLines}&\Use{dyad_7fc140SyntacticTime}&\Use{dyad_7fc140SemanticTime}\\
\Use{dyad_860e21Name}&\Use{dyad_860e21ChangeSize}&\Use{dyad_860e21SyntacticLines}&\Use{dyad_860e21SemanticLines}&\Use{dyad_860e21SyntacticTime}&\Use{dyad_860e21SemanticTime}\\
\Use{dyad_9202b9Name}&\Use{dyad_9202b9ChangeSize}&\Use{dyad_9202b9SyntacticLines}&\Use{dyad_9202b9SemanticLines}&\Use{dyad_9202b9SyntacticTime}&\Use{dyad_9202b9SemanticTime}\\
\Use{dyad_948e6fName}&\Use{dyad_948e6fChangeSize}&\Use{dyad_948e6fSyntacticLines}&\Use{dyad_948e6fSemanticLines}&\Use{dyad_948e6fSyntacticTime}&\Use{dyad_948e6fSemanticTime}\\
\Use{dyad_a540bfName}&\Use{dyad_a540bfChangeSize}&\Use{dyad_a540bfSyntacticLines}&\Use{dyad_a540bfSemanticLines}&\Use{dyad_a540bfSyntacticTime}&\Use{dyad_a540bfSemanticTime}\\
\Use{dyad_abd2aeName}&\Use{dyad_abd2aeChangeSize}&\Use{dyad_abd2aeSyntacticLines}&\Use{dyad_abd2aeSemanticLines}&\Use{dyad_abd2aeSyntacticTime}&\Use{dyad_abd2aeSemanticTime}\\
\Use{dyad_b1a4a7Name}&\Use{dyad_b1a4a7ChangeSize}&\Use{dyad_b1a4a7SyntacticLines}&\Use{dyad_b1a4a7SemanticLines}&\Use{dyad_b1a4a7SyntacticTime}&\Use{dyad_b1a4a7SemanticTime}\\
\Use{tinyvm_378cc6Name}&\Use{tinyvm_378cc6ChangeSize}&\Use{tinyvm_378cc6SyntacticLines}&\Use{tinyvm_378cc6SemanticLines}&\Use{tinyvm_378cc6SyntacticTime}&\Use{tinyvm_378cc6SemanticTime}\\
\Use{dyad_b1a4a7Name}&\Use{dyad_b1a4a7ChangeSize}&\Use{dyad_b1a4a7SyntacticLines}&\Use{dyad_b1a4a7SemanticLines}&\Use{dyad_b1a4a7SyntacticTime}&\Use{dyad_b1a4a7SemanticTime}\\
\Use{dyad_c5e4b5Name}&\Use{dyad_c5e4b5ChangeSize}&\Use{dyad_c5e4b5SyntacticLines}&\Use{dyad_c5e4b5SemanticLines}&\Use{dyad_c5e4b5SyntacticTime}&\Use{dyad_c5e4b5SemanticTime}\\
\Use{dyad_fca75eName}&\Use{dyad_fca75eChangeSize}&\Use{dyad_fca75eSyntacticLines}&\Use{dyad_fca75eSemanticLines}&\Use{dyad_fca75eSyntacticTime}&\Use{dyad_fca75eSemanticTime}\\
\Use{flingfd_0be46bName}&\Use{flingfd_0be46bChangeSize}&\Use{flingfd_0be46bSyntacticLines}&\Use{flingfd_0be46bSemanticLines}&\Use{flingfd_0be46bSyntacticTime}&\Use{flingfd_0be46bSemanticTime}\\
\Use{mdp_004704Name}&\Use{mdp_004704ChangeSize}&\Use{mdp_004704SyntacticLines}&\Use{mdp_004704SemanticLines}&\Use{mdp_004704SyntacticTime}&\Use{mdp_004704SemanticTime}\\
\Use{mdp_00c2adName}&\Use{mdp_00c2adChangeSize}&\Use{mdp_00c2adSyntacticLines}&\Use{mdp_00c2adSemanticLines}&\Use{mdp_00c2adSyntacticTime}&\Use{mdp_00c2adSemanticTime}\\
\Use{mdp_0871e1Name}&\Use{mdp_0871e1ChangeSize}&\Use{mdp_0871e1SyntacticLines}&\Use{mdp_0871e1SemanticLines}&\Use{mdp_0871e1SyntacticTime}&\Use{mdp_0871e1SemanticTime}\\
\Use{mdp_1dfc0dName}&\Use{mdp_1dfc0dChangeSize}&\Use{mdp_1dfc0dSyntacticLines}&\Use{mdp_1dfc0dSemanticLines}&\Use{mdp_1dfc0dSyntacticTime}&\Use{mdp_1dfc0dSemanticTime}\\
\Use{mdp_24fbdfName}&\Use{mdp_24fbdfChangeSize}&\Use{mdp_24fbdfSyntacticLines}&\Use{mdp_24fbdfSemanticLines}&\Use{mdp_24fbdfSyntacticTime}&\Use{mdp_24fbdfSemanticTime}\\
\Use{mdp_2dcbfdName}&\Use{mdp_2dcbfdChangeSize}&\Use{mdp_2dcbfdSyntacticLines}&\Use{mdp_2dcbfdSemanticLines}&\Use{mdp_2dcbfdSyntacticTime}&\Use{mdp_2dcbfdSemanticTime}\\
\Use{mdp_455a6aName}&\Use{mdp_455a6aChangeSize}&\Use{mdp_455a6aSyntacticLines}&\Use{mdp_455a6aSemanticLines}&\Use{mdp_455a6aSyntacticTime}&\Use{mdp_455a6aSemanticTime}\\
\Use{mdp_4f50d6Name}&\Use{mdp_4f50d6ChangeSize}&\Use{mdp_4f50d6SyntacticLines}&\Use{mdp_4f50d6SemanticLines}&\Use{mdp_4f50d6SyntacticTime}&\Use{mdp_4f50d6SemanticTime}\\
\Use{mdp_51b2a8Name}&\Use{mdp_51b2a8ChangeSize}&\Use{mdp_51b2a8SyntacticLines}&\Use{mdp_51b2a8SemanticLines}&\Use{mdp_51b2a8SyntacticTime}&\Use{mdp_51b2a8SemanticTime}\\
\Use{mdp_549e0bName}&\Use{mdp_549e0bChangeSize}&\Use{mdp_549e0bSyntacticLines}&\Use{mdp_549e0bSemanticLines}&\Use{mdp_549e0bSyntacticTime}&\Use{mdp_549e0bSemanticTime}\\
\Use{mdp_58e631Name}&\Use{mdp_58e631ChangeSize}&\Use{mdp_58e631SyntacticLines}&\Use{mdp_58e631SemanticLines}&\Use{mdp_58e631SyntacticTime}&\Use{mdp_58e631SemanticTime}\\
\Use{mdp_629c2eName}&\Use{mdp_629c2eChangeSize}&\Use{mdp_629c2eSyntacticLines}&\Use{mdp_629c2eSemanticLines}&\Use{mdp_629c2eSyntacticTime}&\Use{mdp_629c2eSemanticTime}\\
\Use{mdp_65f9a2Name}&\Use{mdp_65f9a2ChangeSize}&\Use{mdp_65f9a2SyntacticLines}&\Use{mdp_65f9a2SemanticLines}&\Use{mdp_65f9a2SyntacticTime}&\Use{mdp_65f9a2SemanticTime}\\
\Use{mdp_698e2fName}&\Use{mdp_698e2fChangeSize}&\Use{mdp_698e2fSyntacticLines}&\Use{mdp_698e2fSemanticLines}&\Use{mdp_698e2fSyntacticTime}&\Use{mdp_698e2fSemanticTime}\\
\Use{mdp_6d8a33Name}&\Use{mdp_6d8a33ChangeSize}&\Use{mdp_6d8a33SyntacticLines}&\Use{mdp_6d8a33SemanticLines}&\Use{mdp_6d8a33SyntacticTime}&\Use{mdp_6d8a33SemanticTime}\\
\Use{mdp_707f12Name}&\Use{mdp_707f12ChangeSize}&\Use{mdp_707f12SyntacticLines}&\Use{mdp_707f12SemanticLines}&\Use{mdp_707f12SyntacticTime}&\Use{mdp_707f12SemanticTime}\\
\Use{mdp_74ee02Name}&\Use{mdp_74ee02ChangeSize}&\Use{mdp_74ee02SyntacticLines}&\Use{mdp_74ee02SemanticLines}&\Use{mdp_74ee02SyntacticTime}&\Use{mdp_74ee02SemanticTime}\\
\Use{mdp_7b546fName}&\Use{mdp_7b546fChangeSize}&\Use{mdp_7b546fSyntacticLines}&\Use{mdp_7b546fSemanticLines}&\Use{mdp_7b546fSyntacticTime}&\Use{mdp_7b546fSemanticTime}\\
\Use{mdp_7eb09dName}&\Use{mdp_7eb09dChangeSize}&\Use{mdp_7eb09dSyntacticLines}&\Use{mdp_7eb09dSemanticLines}&\Use{mdp_7eb09dSyntacticTime}&\Use{mdp_7eb09dSemanticTime}\\
\Use{mdp_a64de8Name}&\Use{mdp_a64de8ChangeSize}&\Use{mdp_a64de8SyntacticLines}&\Use{mdp_a64de8SemanticLines}&\Use{mdp_a64de8SyntacticTime}&\Use{mdp_a64de8SemanticTime}\\
\Use{mdp_afbf5eName}&\Use{mdp_afbf5eChangeSize}&\Use{mdp_afbf5eSyntacticLines}&\Use{mdp_afbf5eSemanticLines}&\Use{mdp_afbf5eSyntacticTime}&\Use{mdp_afbf5eSemanticTime}\\
\Use{mdp_b19204Name}&\Use{mdp_b19204ChangeSize}&\Use{mdp_b19204SyntacticLines}&\Use{mdp_b19204SemanticLines}&\Use{mdp_b19204SyntacticTime}&\Use{mdp_b19204SemanticTime}\\
\Use{mdp_d00649Name}&\Use{mdp_d00649ChangeSize}&\Use{mdp_d00649SyntacticLines}&\Use{mdp_d00649SemanticLines}&\Use{mdp_d00649SyntacticTime}&\Use{mdp_d00649SemanticTime}\\
\Use{mdp_d35a52Name}&\Use{mdp_d35a52ChangeSize}&\Use{mdp_d35a52SyntacticLines}&\Use{mdp_d35a52SemanticLines}&\Use{mdp_d35a52SyntacticTime}&\Use{mdp_d35a52SemanticTime}\\
\Use{mdp_d83469Name}&\Use{mdp_d83469ChangeSize}&\Use{mdp_d83469SyntacticLines}&\Use{mdp_d83469SemanticLines}&\Use{mdp_d83469SyntacticTime}&\Use{mdp_d83469SemanticTime}\\
\Use{mdp_e2f5b3Name}&\Use{mdp_e2f5b3ChangeSize}&\Use{mdp_e2f5b3SyntacticLines}&\Use{mdp_e2f5b3SemanticLines}&\Use{mdp_e2f5b3SyntacticTime}&\Use{mdp_e2f5b3SemanticTime}\\
\Use{mdp_f6eba2Name}&\Use{mdp_f6eba2ChangeSize}&\Use{mdp_f6eba2SyntacticLines}&\Use{mdp_f6eba2SemanticLines}&\Use{mdp_f6eba2SyntacticTime}&\Use{mdp_f6eba2SemanticTime}\\
\Use{mdp_fc7c1dName}&\Use{mdp_fc7c1dChangeSize}&\Use{mdp_fc7c1dSyntacticLines}&\Use{mdp_fc7c1dSemanticLines}&\Use{mdp_fc7c1dSyntacticTime}&\Use{mdp_fc7c1dSemanticTime}\\
\Use{siemens_print_tokens2Name}&\Use{siemens_print_tokens2ChangeSize}&\Use{siemens_print_tokens2SyntacticLines}&\Use{siemens_print_tokens2SemanticLines}&\Use{siemens_print_tokens2SyntacticTime}&\Use{siemens_print_tokens2SemanticTime}\\
\Use{siemens_print_tokens2Name}&\Use{siemens_print_tokens2ChangeSize}&\Use{siemens_print_tokens2SyntacticLines}&\Use{siemens_print_tokens2SemanticLines}&\Use{siemens_print_tokens2SyntacticTime}&\Use{siemens_print_tokens2SemanticTime}\\
\Use{siemens_print_tokens2Name}&\Use{siemens_print_tokens2ChangeSize}&\Use{siemens_print_tokens2SyntacticLines}&\Use{siemens_print_tokens2SemanticLines}&\Use{siemens_print_tokens2SyntacticTime}&\Use{siemens_print_tokens2SemanticTime}\\
\Use{siemens_print_tokens2Name}&\Use{siemens_print_tokens2ChangeSize}&\Use{siemens_print_tokens2SyntacticLines}&\Use{siemens_print_tokens2SemanticLines}&\Use{siemens_print_tokens2SyntacticTime}&\Use{siemens_print_tokens2SemanticTime}\\
\Use{siemens_print_tokens2Name}&\Use{siemens_print_tokens2ChangeSize}&\Use{siemens_print_tokens2SyntacticLines}&\Use{siemens_print_tokens2SemanticLines}&\Use{siemens_print_tokens2SyntacticTime}&\Use{siemens_print_tokens2SemanticTime}\\
\Use{siemens_print_tokens2Name}&\Use{siemens_print_tokens2ChangeSize}&\Use{siemens_print_tokens2SyntacticLines}&\Use{siemens_print_tokens2SemanticLines}&\Use{siemens_print_tokens2SyntacticTime}&\Use{siemens_print_tokens2SemanticTime}\\
\Use{siemens_print_tokens2Name}&\Use{siemens_print_tokens2ChangeSize}&\Use{siemens_print_tokens2SyntacticLines}&\Use{siemens_print_tokens2SemanticLines}&\Use{siemens_print_tokens2SyntacticTime}&\Use{siemens_print_tokens2SemanticTime}\\
\Use{siemens_print_tokens2Name}&\Use{siemens_print_tokens2ChangeSize}&\Use{siemens_print_tokens2SyntacticLines}&\Use{siemens_print_tokens2SemanticLines}&\Use{siemens_print_tokens2SyntacticTime}&\Use{siemens_print_tokens2SemanticTime}\\
\Use{siemens_print_tokens2Name}&\Use{siemens_print_tokens2ChangeSize}&\Use{siemens_print_tokens2SyntacticLines}&\Use{siemens_print_tokens2SemanticLines}&\Use{siemens_print_tokens2SyntacticTime}&\Use{siemens_print_tokens2SemanticTime}\\
\Use{siemens_print_tokens2Name}&\Use{siemens_print_tokens2ChangeSize}&\Use{siemens_print_tokens2SyntacticLines}&\Use{siemens_print_tokens2SemanticLines}&\Use{siemens_print_tokens2SyntacticTime}&\Use{siemens_print_tokens2SemanticTime}\\
\Use{siemens_print_tokensName}&\Use{siemens_print_tokensChangeSize}&\Use{siemens_print_tokensSyntacticLines}&\Use{siemens_print_tokensSemanticLines}&\Use{siemens_print_tokensSyntacticTime}&\Use{siemens_print_tokensSemanticTime}\\
\Use{siemens_print_tokensName}&\Use{siemens_print_tokensChangeSize}&\Use{siemens_print_tokensSyntacticLines}&\Use{siemens_print_tokensSemanticLines}&\Use{siemens_print_tokensSyntacticTime}&\Use{siemens_print_tokensSemanticTime}\\
\Use{siemens_print_tokensName}&\Use{siemens_print_tokensChangeSize}&\Use{siemens_print_tokensSyntacticLines}&\Use{siemens_print_tokensSemanticLines}&\Use{siemens_print_tokensSyntacticTime}&\Use{siemens_print_tokensSemanticTime}\\
\Use{siemens_print_tokensName}&\Use{siemens_print_tokensChangeSize}&\Use{siemens_print_tokensSyntacticLines}&\Use{siemens_print_tokensSemanticLines}&\Use{siemens_print_tokensSyntacticTime}&\Use{siemens_print_tokensSemanticTime}\\
\Use{siemens_print_tokensName}&\Use{siemens_print_tokensChangeSize}&\Use{siemens_print_tokensSyntacticLines}&\Use{siemens_print_tokensSemanticLines}&\Use{siemens_print_tokensSyntacticTime}&\Use{siemens_print_tokensSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_replaceName}&\Use{siemens_replaceChangeSize}&\Use{siemens_replaceSyntacticLines}&\Use{siemens_replaceSemanticLines}&\Use{siemens_replaceSyntacticTime}&\Use{siemens_replaceSemanticTime}\\
\Use{siemens_scheduleName}&\Use{siemens_scheduleChangeSize}&\Use{siemens_scheduleSyntacticLines}&\Use{siemens_scheduleSemanticLines}&\Use{siemens_scheduleSyntacticTime}&\Use{siemens_scheduleSemanticTime}\\
\Use{siemens_scheduleName}&\Use{siemens_scheduleChangeSize}&\Use{siemens_scheduleSyntacticLines}&\Use{siemens_scheduleSemanticLines}&\Use{siemens_scheduleSyntacticTime}&\Use{siemens_scheduleSemanticTime}\\
\Use{siemens_scheduleName}&\Use{siemens_scheduleChangeSize}&\Use{siemens_scheduleSyntacticLines}&\Use{siemens_scheduleSemanticLines}&\Use{siemens_scheduleSyntacticTime}&\Use{siemens_scheduleSemanticTime}\\
\Use{siemens_scheduleName}&\Use{siemens_scheduleChangeSize}&\Use{siemens_scheduleSyntacticLines}&\Use{siemens_scheduleSemanticLines}&\Use{siemens_scheduleSyntacticTime}&\Use{siemens_scheduleSemanticTime}\\
\Use{siemens_scheduleName}&\Use{siemens_scheduleChangeSize}&\Use{siemens_scheduleSyntacticLines}&\Use{siemens_scheduleSemanticLines}&\Use{siemens_scheduleSyntacticTime}&\Use{siemens_scheduleSemanticTime}\\
\Use{siemens_scheduleName}&\Use{siemens_scheduleChangeSize}&\Use{siemens_scheduleSyntacticLines}&\Use{siemens_scheduleSemanticLines}&\Use{siemens_scheduleSyntacticTime}&\Use{siemens_scheduleSemanticTime}\\
\Use{siemens_scheduleName}&\Use{siemens_scheduleChangeSize}&\Use{siemens_scheduleSyntacticLines}&\Use{siemens_scheduleSemanticLines}&\Use{siemens_scheduleSyntacticTime}&\Use{siemens_scheduleSemanticTime}\\
\Use{siemens_scheduleName}&\Use{siemens_scheduleChangeSize}&\Use{siemens_scheduleSyntacticLines}&\Use{siemens_scheduleSemanticLines}&\Use{siemens_scheduleSyntacticTime}&\Use{siemens_scheduleSemanticTime}\\
\Use{siemens_scheduleName}&\Use{siemens_scheduleChangeSize}&\Use{siemens_scheduleSyntacticLines}&\Use{siemens_scheduleSemanticLines}&\Use{siemens_scheduleSyntacticTime}&\Use{siemens_scheduleSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tcasName}&\Use{siemens_tcasChangeSize}&\Use{siemens_tcasSyntacticLines}&\Use{siemens_tcasSemanticLines}&\Use{siemens_tcasSyntacticTime}&\Use{siemens_tcasSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{siemens_tot_infoName}&\Use{siemens_tot_infoChangeSize}&\Use{siemens_tot_infoSyntacticLines}&\Use{siemens_tot_infoSemanticLines}&\Use{siemens_tot_infoSyntacticTime}&\Use{siemens_tot_infoSemanticTime}\\
\Use{spaceName}&\Use{spaceChangeSize}&\Use{spaceSyntacticLines}&\Use{spaceSemanticLines}&\Use{spaceSyntacticTime}&\Use{spaceSemanticTime}\\
\Use{spaceName}&\Use{spaceChangeSize}&\Use{spaceSyntacticLines}&\Use{spaceSemanticLines}&\Use{spaceSyntacticTime}&\Use{spaceSemanticTime}\\
\Use{spaceName}&\Use{spaceChangeSize}&\Use{spaceSyntacticLines}&\Use{spaceSemanticLines}&\Use{spaceSyntacticTime}&\Use{spaceSemanticTime}\\
\Use{theft_4a5aeeName}&\Use{theft_4a5aeeChangeSize}&\Use{theft_4a5aeeSyntacticLines}&\Use{theft_4a5aeeSemanticLines}&\Use{theft_4a5aeeSyntacticTime}&\Use{theft_4a5aeeSemanticTime}\\
\Use{theft_5ace67Name}&\Use{theft_5ace67ChangeSize}&\Use{theft_5ace67SyntacticLines}&\Use{theft_5ace67SemanticLines}&\Use{theft_5ace67SyntacticTime}&\Use{theft_5ace67SemanticTime}\\
\Use{tinyvm_07c32bName}&\Use{tinyvm_07c32bChangeSize}&\Use{tinyvm_07c32bSyntacticLines}&\Use{tinyvm_07c32bSemanticLines}&\Use{tinyvm_07c32bSyntacticTime}&\Use{tinyvm_07c32bSemanticTime}\\
\Use{tinyvm_0dcbd9Name}&\Use{tinyvm_0dcbd9ChangeSize}&\Use{tinyvm_0dcbd9SyntacticLines}&\Use{tinyvm_0dcbd9SemanticLines}&\Use{tinyvm_0dcbd9SyntacticTime}&\Use{tinyvm_0dcbd9SemanticTime}\\
\Use{tinyvm_279bdcName}&\Use{tinyvm_279bdcChangeSize}&\Use{tinyvm_279bdcSyntacticLines}&\Use{tinyvm_279bdcSemanticLines}&\Use{tinyvm_279bdcSyntacticTime}&\Use{tinyvm_279bdcSemanticTime}\\
\Use{tinyvm_27cde3Name}&\Use{tinyvm_27cde3ChangeSize}&\Use{tinyvm_27cde3SyntacticLines}&\Use{tinyvm_27cde3SemanticLines}&\Use{tinyvm_27cde3SyntacticTime}&\Use{tinyvm_27cde3SemanticTime}\\
\Use{tinyvm_4c7363Name}&\Use{tinyvm_4c7363ChangeSize}&\Use{tinyvm_4c7363SyntacticLines}&\Use{tinyvm_4c7363SemanticLines}&\Use{tinyvm_4c7363SyntacticTime}&\Use{tinyvm_4c7363SemanticTime}\\
\Use{tinyvm_595f3eName}&\Use{tinyvm_595f3eChangeSize}&\Use{tinyvm_595f3eSyntacticLines}&\Use{tinyvm_595f3eSemanticLines}&\Use{tinyvm_595f3eSyntacticTime}&\Use{tinyvm_595f3eSemanticTime}\\
\Use{tinyvm_607c7eName}&\Use{tinyvm_607c7eChangeSize}&\Use{tinyvm_607c7eSyntacticLines}&\Use{tinyvm_607c7eSemanticLines}&\Use{tinyvm_607c7eSyntacticTime}&\Use{tinyvm_607c7eSemanticTime}\\
\Use{tinyvm_64edf5Name}&\Use{tinyvm_64edf5ChangeSize}&\Use{tinyvm_64edf5SyntacticLines}&\Use{tinyvm_64edf5SemanticLines}&\Use{tinyvm_64edf5SyntacticTime}&\Use{tinyvm_64edf5SemanticTime}\\
\Use{tinyvm_716936Name}&\Use{tinyvm_716936ChangeSize}&\Use{tinyvm_716936SyntacticLines}&\Use{tinyvm_716936SemanticLines}&\Use{tinyvm_716936SyntacticTime}&\Use{tinyvm_716936SemanticTime}\\
\Use{tinyvm_7dd5a0Name}&\Use{tinyvm_7dd5a0ChangeSize}&\Use{tinyvm_7dd5a0SyntacticLines}&\Use{tinyvm_7dd5a0SemanticLines}&\Use{tinyvm_7dd5a0SyntacticTime}&\Use{tinyvm_7dd5a0SemanticTime}\\
\Use{tinyvm_9694e3Name}&\Use{tinyvm_9694e3ChangeSize}&\Use{tinyvm_9694e3SyntacticLines}&\Use{tinyvm_9694e3SemanticLines}&\Use{tinyvm_9694e3SyntacticTime}&\Use{tinyvm_9694e3SemanticTime}\\
\Use{tinyvm_977111Name}&\Use{tinyvm_977111ChangeSize}&\Use{tinyvm_977111SyntacticLines}&\Use{tinyvm_977111SemanticLines}&\Use{tinyvm_977111SyntacticTime}&\Use{tinyvm_977111SemanticTime}\\
\Use{tinyvm_9f563aName}&\Use{tinyvm_9f563aChangeSize}&\Use{tinyvm_9f563aSyntacticLines}&\Use{tinyvm_9f563aSemanticLines}&\Use{tinyvm_9f563aSyntacticTime}&\Use{tinyvm_9f563aSemanticTime}\\
\Use{tinyvm_aa57b0Name}&\Use{tinyvm_aa57b0ChangeSize}&\Use{tinyvm_aa57b0SyntacticLines}&\Use{tinyvm_aa57b0SemanticLines}&\Use{tinyvm_aa57b0SyntacticTime}&\Use{tinyvm_aa57b0SemanticTime}\\
\Use{tinyvm_af62b0Name}&\Use{tinyvm_af62b0ChangeSize}&\Use{tinyvm_af62b0SyntacticLines}&\Use{tinyvm_af62b0SemanticLines}&\Use{tinyvm_af62b0SyntacticTime}&\Use{tinyvm_af62b0SemanticTime}\\
\Use{tinyvm_af76c4Name}&\Use{tinyvm_af76c4ChangeSize}&\Use{tinyvm_af76c4SyntacticLines}&\Use{tinyvm_af76c4SemanticLines}&\Use{tinyvm_af76c4SyntacticTime}&\Use{tinyvm_af76c4SemanticTime}\\
\Use{tinyvm_c6219fName}&\Use{tinyvm_c6219fChangeSize}&\Use{tinyvm_c6219fSyntacticLines}&\Use{tinyvm_c6219fSemanticLines}&\Use{tinyvm_c6219fSyntacticTime}&\Use{tinyvm_c6219fSemanticTime}\\
\Use{tinyvm_cc99ecName}&\Use{tinyvm_cc99ecChangeSize}&\Use{tinyvm_cc99ecSyntacticLines}&\Use{tinyvm_cc99ecSemanticLines}&\Use{tinyvm_cc99ecSyntacticTime}&\Use{tinyvm_cc99ecSemanticTime}\\
\Use{tinyvm_d15275Name}&\Use{tinyvm_d15275ChangeSize}&\Use{tinyvm_d15275SyntacticLines}&\Use{tinyvm_d15275SemanticLines}&\Use{tinyvm_d15275SyntacticTime}&\Use{tinyvm_d15275SemanticTime}\\
\Use{tinyvm_e6d9d9Name}&\Use{tinyvm_e6d9d9ChangeSize}&\Use{tinyvm_e6d9d9SyntacticLines}&\Use{tinyvm_e6d9d9SemanticLines}&\Use{tinyvm_e6d9d9SyntacticTime}&\Use{tinyvm_e6d9d9SemanticTime}\\
\Use{tinyvm_eb5b16Name}&\Use{tinyvm_eb5b16ChangeSize}&\Use{tinyvm_eb5b16SyntacticLines}&\Use{tinyvm_eb5b16SemanticLines}&\Use{tinyvm_eb5b16SyntacticTime}&\Use{tinyvm_eb5b16SemanticTime}\\
\Use{tinyvm_f60fb7Name}&\Use{tinyvm_f60fb7ChangeSize}&\Use{tinyvm_f60fb7SyntacticLines}&\Use{tinyvm_f60fb7SemanticLines}&\Use{tinyvm_f60fb7SyntacticTime}&\Use{tinyvm_f60fb7SemanticTime}\\
\bottomrule
\end{tabular}
\caption{Results}
\label{fig:summary}
\end{center}
\end{figure*}


